Enforcing Almost-Sure Reachability in POMDPs

Partially-Observable Markov Decision Processes (POMDPs) are a well-known stochastic model for sequential decision making under limited information. We consider the EXPTIME-hard problem of synthesising policies that almost-surely reach some goal state without ever visiting a bad state. In particular, we are interested in computing the winning region, that is, the set of system configurations from which a policy exists that satisfies the reachability specification. A direct application of such a winning region is the safe exploration of POMDPs by, for instance, restricting the behavior of a reinforcement learning agent to the region. We present two algorithms: A novel SAT-based iterative approach and a decision-diagram based alternative. The empirical evaluation demonstrates the feasibility and efficacy of the approaches.

==> impact.tex <==
%

%\section*{Ethics Statement}
%POMDPs are widely used as a model for planning and decision making in various application domains
%of societal importance, including transportation and healthcare. Reach-avoid specifications have a particularly
%important application in robot path planning and navigation. Similarly our work contributes towards the topic of 
%safe reinforcement learning (RL) which is important given the growing applications for RL. By providing strong 
%guarantees about the correctness of generated policies, this work contributes towards improving the dependability 
%of systems in these domains.
%
%We are also aware that due to the generality of POMDPs, people with malicious intent may use planning under
%uncertainty for malicious purposes. At this stage, we do not know of a way in which such activities can be prevented.
%Nevertheless, we hope that our research, together with the publicly available source code, can help strengthen
%the safety and dependability of technologies that are in the interest of society.
 

==> pics/pomdp_ex.tex <==
\begin{tikzpicture}
\node[fill=obs1, state, circle] (s1) {$s_1$};
\node[fill, circle, right=0.8cm of s1, yshift=1cm] (s1a1) {};

\node[fill=obs2, state,below=\verticaldistance of s1, xshift=\horizontaldistance] (s2) {$s_2$};
\node[fill=obs3, state,above=\verticaldistance of s1, xshift=\horizontaldistance*2] (s3) {$s_3$};
\node[fill=obs3, state,below=\verticaldistance of s1, xshift=\horizontaldistance*2] (s4) {$s_4$};
\node[fill, circle, above=0.8cm of s4] (s4a2) {};

\node[fill=reach, state,above=\verticaldistance of s1, xshift=\horizontaldistance*3] (r) {$R$};
\node[fill=avoid, state,below=\verticaldistance of s1, xshift=\horizontaldistance*3] (a) {$A$};

\draw ($(s1.west) - (0.3,0)$) edge[->] (s1);
\draw[thick] (s1) edge node[above=0.2cm,near start] {$\alpha$} (s1a1);
\draw[->,thick] (s1) edge node[above=0.2cm] {$\beta$} (s2);
%
\draw[->] (s1a1) edge node[above, near start] {\scriptsize$0.5$} (s3);
\draw[->] (s1a1) edge node[below=0.2cm, near start] {\scriptsize$0.5$} (s4);

\draw[->,thick] (s2) edge [bend left] node[below=0.2cm, near start] {$\beta$} (s1);
\draw[->,thick] (s2) edge [] node[above, near start] {$\alpha$} (s4);


\draw[->,thick] (s3) edge [] node[above] {$\alpha$} (r);
\draw[->,thick] (s3) edge [] node[left, near start] {$\beta$} (s2);


\draw[->,thick] (s4) edge [] node[above] {$\alpha$} (a);
\draw[thick] (s4) edge node[left] {$\beta$} (s4a2);
\draw[->] (s4a2) edge node[left, near start] {\scriptsize$0.1$} (s3);
\draw[->] (s4a2) edge [bend left] node[right, near start] {\scriptsize$0.9$} (s4);



\end{tikzpicture}




==> pics/pomdp_ex_bsmdp.tex <==
\begin{tikzpicture}
\node[fill=obs1, state, circle, minimum size=10mm] (s1) {$s_1$};

\node[fill=obs2, state,below=\verticaldistance of s1, xshift=\horizontaldistance] (s2) {$s_2$};
\node[fill=obs3, state,above=\verticaldistance of s1, xshift=\horizontaldistance, minimum size=10mm, inner sep=-1mm] (s34) {$s_3,s_4$};
\node[fill, circle, right=0.8cm of s34] (s34a1) {};
\node[fill, circle, below=0.8cm of s34,xshift=1.2cm] (s34a2) {};

\node[fill=reach, state,above=\verticaldistance of s1, xshift=\horizontaldistance*3, minimum size=10mm] (r) {$R$};
\node[fill=avoid, state,below=\verticaldistance of s1, xshift=\horizontaldistance*3] (a) {$A$};

\draw ($(s1.west) - (0.3,0)$) edge[->] (s1);
\draw[->,thick] (s1) edge node[above=0.2cm,near start] {$\alpha$} (s34);
\draw[->,thick] (s1) edge node[above=0.2cm] {$\beta$} (s2);
%%
%\draw[->] (s1a1) edge node[above, near start] {\scriptsize$0.5$} (s3);
%\draw[->] (s1a1) edge node[below=0.2cm, near start] {\scriptsize$0.5$} (s4);
%
\draw[->,thick] (s2) edge [bend left] node[below=0.2cm, near start] {$\beta$} (s1);
\draw[->,thick] (s2) edge [] node[left, near start] {$\alpha$} (s34);
%
%
%\draw[->,thick] (s3) edge [] node[above] {$\alpha$} (r);

\draw[thick] (s34) edge node[above] {$\alpha$} (s34a1);
\draw[->] (s34a1) edge node[left, near start] {} (r);
\draw[->] (s34a1) edge [] node[right, near start] {} (a);

\draw[thick] (s34) edge node[left] {$\beta$} (s34a2);
\draw[->] (s34a2) edge node[left, near start] {} (s2);
\draw[->] (s34a2) edge [bend right] node[right, near start] {} (s34);

%\draw[->,thick] (s3) edge [] node[left, near start] {$\beta$} (s2);
%
%
%\draw[->,thick] (s4) edge [] node[above] {$\alpha$} (a);
%


\end{tikzpicture}



